MR-Adopt: Automatic Deduction of Input Transformation Function for Metamorphic Testing

While a recent study reveals that many developer-written test cases can encode a reusable Metamorphic Relation (MR), over 70% of them directly hard-code the source input and follow-up input in the encoded relation. Such encoded MRs, which do not contain an explicit input transformation to transform the source inputs to corresponding follow-up inputs, cannot be reused with new source inputs to enhance test adequacy. In this paper, we propose MR-Adopt (Automatic Deduction Of inPut Transformation) to automatically deduce the input transformation from the hard-coded source and follow-up inputs, aiming to enable the encoded MRs to be reused with new source inputs. With typically only one pair of source and follow-up inputs available in an MR-encoded test case as the example, we leveraged LLMs to understand the intention of the test case and generate additional examples of source-followup input pairs. This helps to guide the generation of input transformations generalizable to multiple source inputs. Besides, to mitigate the issue that LLMs generate erroneous code, we refine LLM-generated transformations by removing MR- irrelevant code elements with data-flow analysis. Finally, we assess candidate transformations based on encoded output relations and select the best transformation as the result. Evaluation results show that MR-Adopt can generate input transformations applicable to all experimental source inputs for 72.00% of encoded MRs, which is 33.33% more than using vanilla GPT-3.5. By incorporating MR- Adopt-generated input transformations, encoded MR-based test cases can effectively enhance the test adequacy, increasing the line coverage and mutation score by 10.62% and 18.91%, respectively.

==> src/glossary.tex <==
% !TeX root = ../main.tex
{\LARGE \textbf{Glossary}}
% \textbf{Table of revision progress: }
% \begin{enumerate}
% \item
% \end{enumerate}
% \newpage

% \textbf{Terminology: } 

\begin{enumerate}[leftmargin=*]

\item introduction:
    \begin{itemize}
      \item tool: \todo{\textsc{MR-Adopt}}: Automatic Deduction Of inPut Transformation
      \item MR \todo{encoded} in test case
      \item Approach: beyond the existing input pair, \tool employs LLMs to digest contextual information and deduce the underlying input relation, and then generate \todo{additional} input pairs as examples to \todo{guide} the generation of \todo{generalizable} input transformations.
      % beyond the existing input pair, contextual information can be leveraged to deduce underlying input relations and generate generalizable transformation functions.
      \item \todo{hardcoded} MRs: MRs whose follow-up inputs are hardcoded.\jr{I am thinking can hardcoded test cases be called MRs? If this term does not appear very often, you may say ``potential MRs with hardcoded inputs'' }\congying{i see, let me check whether it appears very often}
      \item \todo{generalized} MRs: MRs whose follow-up inputs are transformation generated
      %\jr{-aided? -augmented? Prefer shorter terms} OR \todo{generalized} MRs
    \end{itemize}
    
\item methodology:
    \begin{itemize}
      \item Input: a pair of source and follow-up inputs with the context of MR-encoded test case and methods under test.
      \item Output: ``input transformation function(s)'' shorten as \todo{``transformation(s)''}
      \item \phaseOneLong:  \todo{Additional} input pairs will be generated.
      \item \phaseTwoLong: (1) prompt LLMs with multiple concrete input pairs as examples (2) refine LLM's answer by excluding irrelevant code based on \todo{source/follow-up inputs' data-flow path} (3) \todo{assess} the \todo{generalizability} of candidate input transformations
    \end{itemize}
    
\item evaluation: 
    \begin{itemize}
      \item \todo{applicable} transformation: transformations can apply to at least one valid source input in the experiment
      \item \todo{constrained}\jr{overfitting?} transformation: transformation that can apply to part of valid source inputs in the experiment 
      \csq{partially-applicable or sth? since we do not know what is the ``constraint'' to constraint the usage of these MRs. And also, we may not be able to argue that the ITs passing all the generated tests must be generalizable, since these tests may not be adequate (sth like **correct** patches should be evaluated with adequate tests but not only some tests)? We may need to pay attention to this in our evaluation part.}
      \congying{agree. let's choose more appropriate terms.}
      \item \todo{generalizable} transformation: transformation that can apply to all valid source inputs in the experiment


      
      \item \textbf{RQ1:} How effective is \tool in generating input transformations?
    \item \textbf{RQ2:} How effective are \tool-generated input transformations in constructing follow-up inputs, compared to LLMs?
    \item \textbf{RQ3:} What is the contribution of each component in \tool for generating input transformations?
    \item \textbf{RQ4:} How useful are generalized MRs in generating test cases and enhancing test adequacy?
    \end{itemize}
\end{enumerate}

==> src/note.tex <==
% TY CHen: acm survey
The construction of individual test cases is simple. Source
test cases can be generated through existing testing methods, while follow-up test cases can be
constructed through transformations according to MRs.

In particular, it is a very challenging job to propose a specification language that not only supports
the unified expression of MRs by different stakeholders for various purposes but also facilitates
the transformation of individual MRs to a set of automated procedures for constructing MT test
cases, bearing in mind that the follow-up test cases may depend not only on the source test cases
but also on their outputs.

\congying{todo: add example of wrong follow-up date, because of LLMs' limitation in logically reasoning}

update:
summary of RQ4.

==> src/related.tex <==
% !TeX root = ../main.tex

\section{Related Work}

% * Function/program generation (NL->Program/PBE/..)
\subsection{Code generation}

% * MT inputs generation -> : because the research problem changed from MT inputs generation  to input transformation generated
% discuss: how do existing studies construct transformations
% discuss: what are the applications of constructed transformations
\subsection{Input Transformation in MT}

\subsection{MR generation}
TODO, recently LLM-based MR generation work





==> src/revision_response.tex <==
\editedA{
\section{Responses to Meta-review}
}

Dear shepherd and reviewers,

We sincerely appreciate your valuable comments and the opportunity to revise our paper. We have carefully followed your suggestions, and the revised version is attached below, with changes highlighted in blue. We hope this version addresses your concerns, enhances the paper's completeness, and can get your approval.

\textbf{Meta-review Comment: }
"The main condition is for the authors to add a discussion part, comparing with one or two non-MR-tests, and analyzing which kinds of bugs are specific to MR-tests. In addition, the authors shall address the reviewers' comments in the revision as much as possible."

\textbf{Our update: }
To clarify the advantages of MR-based tests in detecting specific faults, we add a new subsection (\textbf{Section 5.2} [L1064-1156@Page10]) in this revision. 
Specifically, we highlight the distinct advantages of MR-based tests in detecting \textbf{faults of ``non-testable'' programs}. 
We compare MR-based tests with two non-MR tests (including developer-written and LLM/EvoSuite-generated tests) in detecting faults in encryption and system time-based programs, which are hard to test since their expected outputs for given inputs are hard to specify. The results demonstrate that MR-based tests can detect the faults that non-MR tests fail to identify.
We also emphasize another advantage of MR-based tests for fault detection: the ability to apply a single MR to a wide range of automatically generated test inputs, thereby exercising diverse program behaviors.

Besides, we have addressed other reviewers' comments in the revision, including: \\
1. Reviewer-A: Clarification on the output relation availability [Section 2.2, L256-261@Page3] \\
2. Reviewer-A: Discussion about the impact of output relations on baseline performances [Section 4.5, L794-799@Page7]\\
3. Reviewer-A: Clarification on the number of examples [Section 3.1, L392-398@Page4]\\
4. Reviewer-B: Details on constructing dependency graphs [Section 3.1, L424-432@Page4] and class name matching in our approach [Section 3.2, L523-554@Page5]\\
5. Reviewer-B: Discussion on handling complex test scenarios with our approach [Section 4.2, L633-638@Page6]\\
6. Reviewer-B: Providing baseline prompts [Section 4.5, L738@Page7] and analysis of Table 3 results [Section 4.7, L918-927@Page8]\\
7. Reviewer-C: Clarification on the creation of new dataset [Section 4.2, L625-628@Page6]\\
8. Reviewer-C: Discussion on the advantages of MR-based tests in fault detection [Section 5.2, L1064-1156@Page10]\\
9. Reviewer-C: Discussion on MR-based tests VS. EvoSuite-generated tests. [Section 5.2, L1136-1156@Page10]

We hope our revisions will get your approval. Once again, thank you very much for your review efforts, as well as your valuable suggestions and comments!

Best regards.

% \csq{Clarification on output relation availability? It is a bit weird to understand "Reviewer A: Refinement ...".}
% \congying{udpated}

==> src/storyline.tex <==
% !TeX root = ../main.tex

{\LARGE \textbf{Story Line}} \\
\congying{this version focuses on the problem in TOSEM paper.}

\textbf{Background.} 
MT is useful, while MR generation is challenging.

Recently, Xu et al. [?] explored discovering and synthesizing executable MRs from existing test cases to facilitate automated MT. \valerio{I think we should say it a bit different, otherwise it seems we are incrementally extending Xu et al. [?]. We should say that Xu et al. [?] shown that there are MR encoded in test cases -> however x\% of them have hard coded values, we need imput transformation to generalise the MR to new inputs. we need to show example here, otherwise the reader is lost  } \congying{[todo] update}

\textbf{Problem.} 
However, lacking input transformation impedes the usage of a large percentage of such encoded MRs.
Deducing input transformations to generalize such MRs to new source inputs.
% \jr{Do you mean impeding the reuse of the mined MRs?}

\textbf{Research challenges and existing work.} 
Constructing transformations is challenging, requiring domain knowledge to understand given MRs and familiarity with related APIs/libraries for implementation. 

In related studies, input transformations were constructed relying on manual effort, and specific to certain domains/ MRs. This suffers from a low degree of automation and is challenging to be widely adopted.
To the best of our knowledge, no approach has been proposed for generating input transformations for MT. 


\textbf{Approach and technical challenges.} 
Recently, LLMs have shown effectiveness in code intention summarization (which reflects the capability to understand the encoded MRs) and code generation (which reflects the capability to generate effective transformations).
\hc{This is too general. We can try to add some elaboration, such as LLMs are trained with lots of code, and it may (to some extent) understand the relationship between domain knowledge and code (i.e., semantics).}
\valerio{I agree is too general, we need to better motivate why LLMs, otherwise seems that we choose LLM because is the new hot thing}
\congying{[todo] add more elaboration.}
In this paper, we propose \tool, an LLM-based approach to automatically generate transformation functions.

\valerio{For a reviewer to understand this challenge, I think more about what our previous technique does.}
\congying{Sorry. Cannot clearly get your point.}
\textbf{Technical challenges.} 
While LLMs have shown effectiveness in common code generation tasks, generating transformation functions for MRs encoded in test cases still has the following challenges:
% \jr{After reading the three bullets, I am not convinced that the challenges are unique to input transformation generation. The overfitting/hallucination/verification problems seem to be general. } \congying{agree. I discard the word ``unique''.}1

\begin{enumerate}
    \item  With only one available input pair for example, how to \textbf{mitigate the overfitting issue and generate a generalizable transformation function?} Our solution: employing LLMs to generate multiple valid input pairs as examples.
    \hc{This is a good one. I like it.}
    \hc{I think we can go beyond the number of input pairs to make this point more interesting. As we discussed in the meeting, for an input relation \(x < y\) one can generate input pairs \((1,2), (1,3), (1, 4)\). However, it is possible that LLMs infer an input relation \(x = y - 1\) and generate input pairs \((1, 2), (2, 3), (3, 4)\). I think there are two levels of overfitting here. One is the input transformation overfits to a specific pair. The other is the input transformation, which represents a relation that is stricter than the expected one. We can dig deeper into this. For example, we introduce some relation relaxation mechanisms.}
    \jr{There is a gap: how can you know the generated examples would fit the ground truth input transformation? Based on the current argument, either (a) generating the transformation directly or (b) first generating more examples, then generating the transformation based on the single example. Maybe we can argue that LLM works better at analogical reasoning. Here is a talk from Sumit Gulwani (a PBE expert): \href{https://www.linkedin.com/feed/update/urn:li:activity:7095272360966041600/}{click me} }
    \congying{interesting. Given the same source input, we can check whether two transformations generate different follow-up inputs. If so, diverse follow-up inputs may exercise different program paths. Our approach can finally output diverse transformations. Let me quickly do some experiments or investigation of dataset.}
    % cannot apply to equivalence relation/reverse relation ... Are applicable MRs prevalent? quickly check the dataset to see the percentage.  
    \item LLMs may produce incorrect inputs/transformation, due to the hallucination issue. how to \textbf{refine LLM-generated incorrect inputs/transformations which just have minor issues} and obtain correct inputs/transformation? \hc{How does hallucination affect the effectiveness? What does refine mean? Why does it help?}
    % \songqiang{How about ``may produce incorrect ITs (due to ...)''?} 
    Our solution: inspired by our observation that LLMs often generate task-irrelevant code segments where errors exist, we design a data-flow analysis-based code refinement strategy to exclude irrelevant code segments from LLM-generated inputs/transformation (and add dependency)
    \jr{So, the refinements we did are removing redundant codes and adding dependencies?}
    \hc{If so, that seems a bit trivial for me.}
    \congying{Thanks for your feedback. Maybe the issue of my tedious presentation. 
    The observation that some errors only exist in redundant code is interesting and novel. If we can extract ``useful'' code only and exclude redundant code, we may get more correct inputs/transformations. (To the best of my knowledge, no one has proposed and utilized such observation.). The technical challenge lays on how to differentiate ``useful'' code from ``redundant'' code, and I choose data-flow analysis to extract code elements used for constructing source/follow-up relevant paths. In other words, considering code elements used for constructing source/follow-up as ``useful'' code.}
    
    \item How to \textbf{automatically validate the generalizability} of generated transformations and select the best one? Our solution: employ LLMs-generated inputs and developer-written output relations as oracles to validate generated transformations.
    \hc{I am thinking if we should try to generate new source inputs with a different input generator. Currently, it sounds like LLM is playing the role of both player and judge.}
    \congying{I think, the keypoint is: ``validation'' step will include more new source inputs that do not appear in the ``transforamtion generation'' step. Because LLMs may not generate valid follow-up inputs for some valid source inputs. Such source inputs can be used for ``validation''' and they are just judge not player. 
    In the evaluation, we will use inputs that do not appear in the methodology.}
    \songqiang{Is this a challenge specific for the evaluation design or also for the methodology?}
    \congying{Both of evaluation and methodology has such challenge. ``Validation'' step in the methodology.}
    \jr{I think the current methodology samples/generates multiple transformations and then selects the ``best'' one?  }\congying{Yes, the current methodology select the best one. And the ranking is based on the generalizability to new source inputs.}
\end{enumerate}



\textbf{Evaluation.} 
% effectiveness
Our evaluation shows the effectiveness of \tool in generating transformations, by comparing with existing code generation approaches (i.e., PBE and prompting LLMs \hc{We are also prompting LLMs aren't we?}).

% necessity
We study the capability of popular LLMs which may serve as universal transformation functions to generate source and corresponding follow-up inputs.
On the one hand, the results indicate the effectiveness of the input generator of \tool in generating several valid input pairs for exampling. On the other hand, the high cost and low success rate \hc{We should have some comparison between our technique and vanilla LLM.} of LLMs motivate the necessity of transformation generation.\jr{Cannot follow this sentence. We also used LLMs. Do you want to compare with using LLMs to generate inputs massively? }

% effectiveness in generating follow-up
Our evaluation shows the effectiveness of transformations generated by \tool in constructing valid follow-up inputs, particularly on source inputs for which LLMs fall short of generating valid follow-up inputs.

% usefulness 
We also demonstrate the usefulness of transformation-based MRs in enhancing test adequacy, by comparing test suites constructed from transformation-based MRs against developer-written test suites and LLM written test suites.


\textbf{Contribution.} 
\begin{itemize}
    \item The first paper focuses on the research problem of input transformation generation, and proposes an approach to automatically generate transformation functions.
    % \item Propose an extensible data-flow analysis based code refinement strategy to mitigate the LLMs’ hallucination issue in code generation \congying{may discard this}. 
    \item \songqiang{(Any interesting solutions for any interesting specific technical challenges?)}\congying{to update}
    \item This paper conducts extensive experiments to evaluate the effectiveness of the \tool in generating transformations, and evaluate the effectiveness and usefulness of generated transformations in constructing follow-up inputs and faculty detection.
    \item The evaluation also studies the capability of the popular LLMs in generating source and follow-up inputs for MT.
    \item We crafted \jr{collected?} a dataset of 100 input transformations, and released the research artifact and all experimental data to facilitate reproduction and follow-up research.
\end{itemize}
